Omnidirectional Wireless Power Transfer with Automatic Power Flow Control

We present an omnidirectional wireless power transfer (WPT) system capable of automatic power flow control using three orthogonal transmitter (Tx)-repeater (Rp) pairs. The power drawn from each transmitter is automatically adjusted depending on the mutual inductance between the receiver and the Tx-Rp pair. The proposed approach enables the receiver to harvest almost uniform power with high efficiency (90\%) regardless of its position.

==> Old versions/equation_try.tex <==
\begin{equation}\label{Eq.Zsimple}
 \begin{bmatrix}
 V_{\rm s}\\ V_{\rm s}\\  V_{\rm s}\\
 0\\ 0\\ 0\\ 0\\
 \end{bmatrix} = 
 \begin{bmatrix}
 R+X_0 & 0     & 0      & \mathrm{j}\omega M_0 & 0 & 0 & \mathrm{j}\omega \gamma_1 M_1 \\
 0     & R+X_0 & 0      & 0 & \mathrm{j}\omega M_0 & 0 & \mathrm{j}\omega \gamma_2 M_2\\
 0     & 0     & R+X_0  & 0 & 0 & \mathrm{j}\omega M_0 & \mathrm{j}\omega \gamma_3 M_3\\
\mathrm{j}\omega M_0  & 0     & 0  & R & 0 & 0 & \mathrm{j}\omega M_1\\
 0     & \mathrm{j}\omega M_0 & 0  & 0 & 0 & \mathrm{j}\omega M_0 & \mathrm{j}\omega M_2\\
 0     &       & \mathrm{j}\omega M_0  & 0 & 0 & \mathrm{j}\omega M_0 & \mathrm{j}\omega M_3\\
 \mathrm{j}\omega \gamma_1 M_1  & \mathrm{j}\omega \gamma_2 M_2 & \mathrm{j}\omega \gamma_3 M_3 & \mathrm{j}\omega  M_1 & \mathrm{j}\omega  M_2 & \mathrm{j}\omega  M_3 & Z_\mathrm{r}
 \end{bmatrix}.
\end{equation}


%--------------------------------------
\begin{equation}\label{Eq.Zsimple}
 \begin{bmatrix}
 R+X_{\rm a} & 0            & 0            & X_0    & 0      & 0      & X_{17} \\
 0           & R+X_{\rm a}  & 0            & 0      & X_0    & 0      & X_{27}\\
 0           & 0            & R+X_{\rm a}  & 0      & 0      & X_0    & X_{37}\\
X_0          & 0            & 0            & R      & 0      & 0      & X_{47}\\
 0           & X_0          & 0            & 0      & R      & 0      & X_{57}\\
 0           & 0            & X_0          & 0      & 0      & R      & X_{67}\\
 X_{17}      & X_{27}       & X_{37}       & X_{47} & X_{57} & X_{67} & R+R_{\rm{L}}
 \end{bmatrix}.
\end{equation}
